On the Riemann-Hilbert problem for a $q$-difference Painlev\'e equation

A Riemann-Hilbert problem for a $q$-difference Painlev\'e equation, known as $q\textrm{P}_{\textrm{IV}}$, is shown to be solvable. This yields a bijective correspondence between the transcendental solutions of $q\textrm{P}_{\textrm{IV}}$ and corresponding data on an associated $q$-monodromy surface. We also construct the moduli space of $q\textrm{P}_{\textrm{IV}}$ explicitly.

==> connection.tex <==
\section{The Nonlinear Connection Problem}
Consider the $q\Pfour$ RHP \ref{prob:RHm} under the following assumptions:
\begin{itemize}
	\item \eqref{eq:asump1} and \eqref{eq:asump2} are satisfied;
	\item the model RHP \ref{prob:RHmodel+inf} has a solution $\Omega(\zeta)$;
	\item the matrix $A_0(\zeta)$, defined in Proposition \ref{prop:rhmodelsystem}, is of the form \eqref{eq:A0form1} for some $r_1,r_2,r_3,\mu_0\in\mathbb{C}^*$ with $r_1r_2r_3=r=qa_0^2a_2i$;
	\item the model RHP \ref{prob:RHmodel-inf} has a solution $\Sigma(\zeta)$;
	\item the matrix $A_\infty(\zeta)$, defined in Proposition \ref{prop:rhmodelsysteminf}, is of the form \eqref{eq:Ainfform1} for some $p_1,p_2,p_3,\mu_\infty\in\mathbb{C}^*$ with $p_1p_2p_3=p=qa_0^2a_2i$.
\end{itemize}
Let $(f^m)_{m\in\mathbb{Z}}$ be the via Theorem \ref{thm:mainresult1} corresponding $q\Pfour(t_0,a)$ transcendent.

Then, on the one hand, Theorem \ref{thm:asymptoticszero} shows that $f^m$ is non-singular for $m\in\mathbb{Z}$ positive large enough, with the following asymptotics near $m=+\infty$,
	\begin{align}
	f_0^{3s+j}&=\sigma_{0,j} t_m^\frac{2}{3}\left(1+\mathcal{O}\left(t_m^\frac{2}{3}\right)\right),\nonumber\\
	f_i^{3s+j}&=\sigma_{i,j} t_m^\frac{2}{3}\left(1+\mathcal{O}\left(t_m^\frac{2}{3}\right)\right),\quad m=3s+j \nonumber\\
	f_2^{3s+j}&=\sigma_{2,j} t_m^\frac{2}{3}\left(1+\mathcal{O}\left(t_m^\frac{2}{3}\right)\right)\nonumber,
	\end{align}
	for fixed $j\in\{0,1,2\}$ as $s\rightarrow +\infty$, where the leading order coefficients are defined by means of
	\begin{equation*}
	r_1=-q\sigma_{2,0}i,\quad r_2=-a_0a_2\sigma_{0,0}i,\quad r_3=-a_0\sigma_{1,0}i
	\end{equation*}
	and equations \eqref{eq:asympsigma}.

On the other hand Theorem \ref{thm:asymptoticsinfty} shows that $f^m$ is non-singular for $m\in\mathbb{Z}$ negative large enough, with the following asymptotics near $m=-\infty$,
		\begin{align}
		f_0^{3s+j}&=\upsilon_{0,j} t_m^\frac{2}{3}+\mathcal{O}(1),\nonumber\\
		f_1^{3s+j}&=\upsilon_{1,j} t_m^\frac{2}{3}+\mathcal{O}(1),\quad m=3s+j \nonumber\\
		f_2^{3s+j}&=\upsilon_{2,j} t_m^\frac{2}{3}+\mathcal{O}(1)\nonumber,
		\end{align}
		for fixed $j\in\{0,1,2\}$ as $s\rightarrow -\infty$, where the leading order coefficients are defined by means of
		\begin{equation*}
		p_1=-q\upsilon_{2,0}^{-1}i,\quad p_2=-a_0a_2\upsilon_{0,0}^{-1}i,\quad p_3=-a_0\upsilon_{1,0}^{-1}i
		\end{equation*}
		and equations \eqref{eq:asympupsilon}.
		
In this case, the nonlinear connection problem translates to the problem of relating the leading order coefficients $\{\sigma_{0,0},\sigma_{1,0},\sigma_{2,0}\}$ near $m=3s=+\infty$ to the leading order coefficients $\{\upsilon_{0,0},\upsilon_{1,0},\upsilon_{2,0}\}$ near $m=3s=-\infty$. By the above, this is equivalent to relating the coefficients $\{r_1,r_2,r_3\}$ of the matrix polynomial $A_0(\zeta)$ to the coefficients $\{p_1,p_2,p_3\}$ of the matrix polynomial $A_\infty(\zeta)$. In turn, by Propositions \ref{prop:rhmodelsystem} and \ref{prop:rhmodelsysteminf} this is equivalent to relating the solution $\Omega(\zeta)$ of RHP problem \ref{prob:RHmodel+inf} to the solution $\Sigma(\zeta)$ of RHP problem \ref{prob:RHmodel-inf}.













